Geant4 simulations of soft proton scattering in X-ray optics. A tentative validation using laboratory measurements

Low energy protons (< 300 keV) can enter the field of view of X-ray space telescopes, scatter at small incident angles, and deposit energy on the detector, causing intense background flares at the focal plane or in the most extreme cases, damaging the X-ray detector. A correct modelization of the physics process responsible for the grazing angle scattering processes is mandatory to evaluate the impact of such events on the performance of future X-ray telescopes as the ESA ATHENA mission. For the first time the Remizovich model, in the approximation of no energy losses, is implemented top of the Geant4 release 10.2. Both the new scattering physics and the built-in Coulomb scattering are used to reproduce the latest experimental results on grazing angle proton scattering. At 250 keV multiple scattering delivers large proton angles and it is not consistent with the observation. Among the tested models, the single scattering seems to better reproduce the scattering efficiency at the three energies but energy loss obtained at small scattering angles is significantly lower than the experimental values. In general, the energy losses obtained in the experiment are higher than what obtained by the simulation. The experimental data are not completely representative of the soft proton scattering experienced by current X-ray telescopes because of the lack of measurements at low energies (< 200 keV) and small reflection angles, so we are not able to address any of the tested models as the one that can certainly reproduce the scattering behavior of low energy protons expected for the ATHENA mission. We can, however, discard multiple scattering as the model able to reproduce soft proton funneling, and affirm that Coulomb single scattering can represent, until further measurements, the best approximation of the proton scattered angular distribution at the exit of X-ray optics.

==> fioretti_biblio.tex <==
\bibitem[\protect\citeauthoryear{Armstrong et al.}{1999}]{arm99}Armstrong T.W. et al., 1999, ``Initial Estimates of Radiation Backgrounds for the Hard X--Ray Telescope on the Planned Constellation--X Mission'', SAIC--TN--99015R3

